COVID-BLUeS -- A Prospective Study on the Value of AI in Lung Ultrasound Analysis

As a lightweight and non-invasive imaging technique, lung ultrasound (LUS) has gained importance for assessing lung pathologies. The use of Artificial intelligence (AI) in medical decision support systems is promising due to the time- and expertise-intensive interpretation, however, due to the poor quality of existing data used for training AI models, their usability for real-world applications remains unclear. In a prospective study, we analyze data from 63 COVID-19 suspects (33 positive) collected at Maastricht University Medical Centre. Ultrasound recordings at six body locations were acquired following the BLUE protocol and manually labeled for severity of lung involvement. Several AI models were applied and trained for detection and severity of pulmonary infection. The severity of the lung infection, as assigned by human annotators based on the LUS videos, is not significantly different between COVID-19 positive and negative patients (p = 0.89). Nevertheless, the predictions of image-based AI models identify a COVID-19 infection with 65% accuracy when applied zero-shot (i.e., trained on other datasets), and up to 79% with targeted training, whereas the accuracy based on human annotations is at most 65%. Multi-modal models combining images and CBC improve significantly over image-only models. Although our analysis generally supports the value of AI in LUS assessment, the evaluated models fall short of the performance expected from previous work. We find this is due to 1) the heterogeneity of LUS datasets, limiting the generalization ability to new data, 2) the frame-based processing of AI models ignoring video-level information, and 3) lack of work on multi-modal models that can extract the most relevant information from video-, image- and variable-based inputs. To aid future research, we publish the dataset at: https://github.com/NinaWie/COVID-BLUES.

==> figures/additional_variables.tex <==

\section{Additional clinical variables}

\begin{table*}
\begin{tabular}{lllll}
\toprule
{} &     Total (n=63) & COVID-19 positive (n=33) & COVID-19 negative (n=30) & p-value for group difference \\
                 &                  &                          &                          &                              \\
\midrule \multicolumn{5}{l}{\textbf{Inclusion criteria}} \\ \midrule 
Fever or chills         &        20 (31\%) &                12 (36\%) &                 8 (26\%) &                         0.58 \\
Cough                   &        39 (61\%) &                22 (66\%) &                17 (56\%) &                         0.58 \\
Difficulty breathing    &        59 (93\%) &                31 (93\%) &                28 (93\%) &                         0.68 \\
Loss of taste           &          3 (4\%) &                  3 (9\%) &                  0 (0\%) &                         0.27 \\
Loss of smell           &          3 (4\%) &                  2 (6\%) &                  1 (3\%) &                         0.93 \\
Sore throat             &          2 (3\%) &                  1 (3\%) &                  1 (3\%) &                         0.52 \\
Congestion              &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Runny nose              &          3 (4\%) &                  1 (3\%) &                  2 (6\%) &                         0.93 \\
\midrule \multicolumn{5}{l}{\textbf{Symptoms}} \\ \midrule 
Earache                 &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Wheezing                &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Joint pain              &          1 (1\%) &                  1 (3\%) &                  0 (0\%) &                         0.96 \\
Dyspnea                 &        56 (88\%) &                30 (90\%) &                26 (86\%) &                         0.89 \\
Decreased consciousness &          1 (1\%) &                  0 (0\%) &                  1 (3\%) &                         0.96 \\
Confusion               &          3 (4\%) &                  3 (9\%) &                  0 (0\%) &                         0.27 \\
Abdominal pain          &          3 (4\%) &                  0 (0\%) &                 3 (10\%) &                         0.20 \\
Nausea                  &        11 (17\%) &                 4 (12\%) &                 7 (23\%) &                         0.40 \\
Vomitting               &         8 (12\%) &                 4 (12\%) &                 4 (13\%) &                         0.81 \\
Diarrhea                &         7 (11\%) &                 5 (15\%) &                  2 (6\%) &                         0.50 \\
Skin rash               &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Lymphadenopathy         &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Ageusia/Dysgeusia       &          4 (6\%) &                 4 (12\%) &                  0 (0\%) &                         0.15 \\
Anosmia/Hyposmia        &          4 (6\%) &                  3 (9\%) &                  1 (3\%) &                         0.68 \\
Emergency case          &        62 (98\%) &                32 (96\%) &               30 (100\%) &                         0.96 \\
\midrule \multicolumn{5}{l}{\textbf{Pulmonary diseases}} \\ \midrule 
DPLD                    &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Cystic fibrosis         &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Pneumothorax            &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Tuberculosis            &  0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &          0.0 ($\pm$ 0.0) &                         1.00 \\
Dyspnea                 &          1 (1\%) &                  0 (0\%) &                  1 (3\%) &                         0.96 \\
Other                   &          2 (3\%) &                  0 (0\%) &                  2 (6\%) &                         0.43 \\
\bottomrule
\end{tabular}
\caption{Additional clinical variables that were removed from \autoref{tab:variables_overview} for the sake of simplicity.}
\end{table*}


==> figures/backup_table_clinical_variables.tex <==
\begin{table}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
            &         
            \begin{tabular}{c} \textbf{Total} \\ \textbf{(n=63)} \end{tabular}
            & \begin{tabular}{c} \textbf{COVID-19-positive}  \\ \textbf{(n=33)} \end{tabular} 
           & \begin{tabular}{c} \textbf{COVID-19-negative } \\ \textbf{(n=30)} \end{tabular}
           & \begin{tabular}{c} \textbf{p-value}  \\ \textbf{(group difference)} \end{tabular} \\
% \multicolumn{5}{l}{\textbf{Blood parameters}} \\ \midrule 
% \midrule \multicolumn{5}{l}{\textbf{History of pulmonary diseases}} \\ \midrule 
% \midrule \multicolumn{5}{l}{\textbf{Vital parameters}} \\ \midrule 
% \midrule \multicolumn{5}{l}{\textbf{Symptoms}} \\ \midrule 
\midrule \multicolumn{5}{l}{\textbf{Patient characteristics}} \\ \midrule 
Age (years)                     &    65.2 ($\pm$ 15.74) &       66.2 ($\pm$ 15.66) &       64.1 ($\pm$ 15.76) &                         0.61 \\
Women                           &             41 (65\%) &                19 (57\%) &                22 (73\%) &                         0.30 \\
Height (cm)                     &    171.7 ($\pm$ 9.36) &       169.8 ($\pm$ 9.26) &       173.7 ($\pm$ 9.05) &                         0.11 \\
Weight (kg)                     &     81.3 ($\pm$ 19.4) &       81.2 ($\pm$ 16.28) &       81.5 ($\pm$ 22.34) &                         0.95 \\
BMI (kg/m2)                     &     27.7 ($\pm$ 6.28) &        28.3 ($\pm$ 5.06) &        27.0 ($\pm$ 7.31) &                         0.44 \\
Smoking                         &             29 (46\%) &                 9 (27\%) &                20 (66\%) &                     < 0.01 (*) \\
\midrule \multicolumn{5}{l}{\textbf{Symptoms}} \\ \midrule 
Fever                           &             21 (33\%) &                13 (39\%) &                 8 (26\%) &                         0.42 \\
Cough                           &             40 (63\%) &                24 (72\%) &                16 (53\%) &                         0.18 \\
Sore throat                     &               3 (4\%) &                  2 (6\%) &                  1 (3\%) &                         0.93 \\
Running nose                    &               4 (6\%) &                  1 (3\%) &                 3 (10\%) &                         0.54 \\
Chest pain                      &             15 (23\%) &                 5 (15\%) &                10 (33\%) &                         0.16 \\
Muscle pain                     &               6 (9\%) &                 6 (18\%) &                  0 (0\%) &                     0.04 (*) \\
Fatigue                         &             13 (20\%) &                10 (30\%) &                 3 (10\%) &                         0.09 \\
Headache                        &              7 (11\%) &                 5 (15\%) &                  2 (6\%) &                         0.50 \\
Number of applying symptoms (max. 8) &      1.7 ($\pm$ 1.27) &         2.1 ($\pm$ 1.42) &         1.2 ($\pm$ 0.85) &                        < 0.01 (*) \\
Duration of symptoms (days)     &    10.6 ($\pm$ 26.49) &         8.1 ($\pm$ 5.12) &       13.4 ($\pm$ 37.86) &                         0.45 \\
\midrule \multicolumn{5}{l}{\textbf{Vital parameters}} \\ \midrule 
Oxygen saturation (\%)          &     92.6 ($\pm$ 4.96) &        90.6 ($\pm$ 4.95) &        94.7 ($\pm$ 4.04) &                     < 0.01  (*) \\
Respiratory rate (/min)         &     21.0 ($\pm$ 5.38) &         22.5 ($\pm$ 4.7) &        19.3 ($\pm$ 5.59) &                     0.02 (*) \\
Pulse (bpm)                     &    92.6 ($\pm$ 21.66) &       95.1 ($\pm$ 21.13) &        89.8 ($\pm$ 21.9) &                         0.35 \\
Body temperature (°C)           &     37.3 ($\pm$ 0.86) &        37.5 ($\pm$ 0.75) &         37.0 ($\pm$ 0.9) &                     0.02 (*) \\
Blood pressure systolic (mmHg)  &   130.7 ($\pm$ 20.11) &      132.7 ($\pm$ 20.31) &      128.5 ($\pm$ 19.65) &                         0.41 \\
Blood pressure diastolic (mmHg) &    78.2 ($\pm$ 14.47) &       79.1 ($\pm$ 11.54) &       77.2 ($\pm$ 17.01) &                         0.62 \\
\midrule \multicolumn{5}{l}{\textbf{History of pulmonary diseases}} \\ \midrule 
Any pulmonary disease           &             36 (57\%) &                19 (57\%) &                17 (56\%) &                         0.86 \\
Asthma                          &               5 (7\%) &                 4 (12\%) &                  1 (3\%) &                         0.41 \\
COPD                            &             13 (20\%) &                 6 (18\%) &                 7 (23\%) &                         0.85 \\
Pneunomia                       &              7 (11\%) &                 4 (12\%) &                 3 (10\%) &                         0.89 \\
Interstitial Lung Disease       &               1 (1\%) &                  1 (3\%) &                  0 (0\%) &                         0.96 \\
\midrule \multicolumn{5}{l}{\textbf{Blood parameters}} \\ \midrule 
pH                              &      7.5 ($\pm$ 0.05) &         7.5 ($\pm$ 0.05) &         7.5 ($\pm$ 0.05) &                         0.34 \\
pCO2 (kPa)                      &       4.4 ($\pm$ 1.0) &         4.3 ($\pm$ 0.54) &         4.6 ($\pm$ 1.34) &                         0.21 \\
p02 (kPa)                       &      9.5 ($\pm$ 2.95) &         9.3 ($\pm$ 2.02) &         9.7 ($\pm$ 3.81) &                         0.62 \\
HC03 (mmol/l)                   &     23.5 ($\pm$ 4.73) &        23.1 ($\pm$ 3.15) &        24.1 ($\pm$ 6.14) &                         0.45 \\
Excess (mmol/l)                 &      0.3 ($\pm$ 4.15) &         0.2 ($\pm$ 3.13) &         0.6 ($\pm$ 5.16) &                         0.75 \\
HG (mmol/l)                     &      8.0 ($\pm$ 1.38) &         8.4 ($\pm$ 0.92) &         7.5 ($\pm$ 1.59) &                     < 0.01 (*) \\
Trombocytes ($10^9/l$)          &  232.8 ($\pm$ 111.99) &     217.6 ($\pm$ 100.05) &     248.0 ($\pm$ 120.88) &                         0.30 \\
Leucocytes ($10^9/l$)           &      9.4 ($\pm$ 9.94) &         7.4 ($\pm$ 3.86) &       11.5 ($\pm$ 13.39) &                         0.10 \\
Lymphocytes ($10^9/l$)          &    17.5 ($\pm$ 15.52) &       14.1 ($\pm$ 10.28) &       21.3 ($\pm$ 19.21) &                         0.09 \\
LDH (U/l)                       &  311.8 ($\pm$ 129.29) &     379.2 ($\pm$ 133.92) &      239.8 ($\pm$ 73.32) &                     < 0.001 (*) \\
CRP (mg/l)                      &    82.2 ($\pm$ 82.55) &      110.4 ($\pm$ 80.14) &       51.2 ($\pm$ 73.58) &                     < 0.01 (*) \\
\bottomrule
\end{tabular}
}
\caption{Overview of clinical variables and their relation to the PCR test result. Data are mean ($\pm$ standard deviation) or n (\%). The significance level of the difference between both groups (positive and negative PCR test) is measured with a Chi-Square test for binary variables and with a t-test for continuous variables (marked with (*) if < 0.05).
% \jb{I would bold each row that is significant and then use stars to indicate the significance level (0.05, 0.01, 0.001).
% Never give p-values of zero, always give exact numbers in scientific notation.
% }
}
\label{tab:variables_overview}
\end{table}




==> figures/table_results_std.tex <==
\begin{table}[h]
\centering
\footnotesize
\setlength{\belowcaptionskip}{-100pt}
\setlength\tabcolsep{2pt}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l}
Model          & \multicolumn{3}{c|}{Images}                                                                              & \multicolumn{3}{c|}{Images and Features}                                                        & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Images and Features \\ without Blood Test\end{tabular}}  \\ 
\hline
               & accuracy                               & sensitivity                    & specificity                    & accuracy                       & sensitivity                   & specificity                    & accuracy                      & sensitivity                    & specificity                           \\ 
\hline
VGG16          & \textbf{73.4\%±5}                      & \textbf{0.90±0.13}             & 0.55±0.24                      & 78.4\%±9                       & 0.87±0.12                     & 0.69±0.19                      & 78.4\%±8                      & 0.77±0.14                      & 0.8±0.12                              \\ 
\hline
ResNet50       & 63.2\%±14                              & 0.77±0.33                      & 0.50±0.35                      & \textbf{80.3\%±13}             & 0.67±0.3                      & \textbf{0.93±0.08}             & \textbf{83.4\%±5}             & \textbf{0.84±0.01}             & 0.83±0.11                             \\ 
\hline
NASNetMobile   & 58.2\%±7                               & 0.61±0.25                      & \textbf{0.90±0.13}             & 78.5\%±17                      & 0.67±0.3                      & 0.9±0.13                       & 75.0\%±17                     & 0.6±0.38                       & \textbf{0.89±0.09}                    \\ 
\hline
MobileNetV2    & 68.4\%±10                              & 0.64±0.2                       & 0.73±0.13                      & 78.4\%±9                       & \textbf{0.88±0.15}            & 0.69±0.22                      & 78.3\%±13                     & 0.7±0.2                        & 0.87±0.12                             \\ 
\hline
EfficientNetB7 & 71.7\%±9                               & 0.77±0.17                      & 0.65±0.25                      & 76.3\%±10                      & 0.64±0.2                      & 0.89±0.09                      & 76.8\%±9                      & 0.81±0.12                      & 0.73±0.27                             \\ 
\hline
Late fusion    & \multicolumn{1}{c|}{\textbf{75.2\%±8}} & \multicolumn{1}{c|}{0.84±0.15} & \multicolumn{1}{c|}{0.65±0.25} & \multicolumn{1}{c|}{76.9\%±16} & \multicolumn{1}{c|}{0.67±0.3} & \multicolumn{1}{c|}{0.87±0.12} & \multicolumn{1}{c|}{80.1\%±8} & \multicolumn{1}{c|}{0.77±0.14} & \multicolumn{1}{c}{0.83±0.11}        
\end{tabular}
\caption{Performance of different network architectures on the three configurations of the dataset together with the standard deviation over the five folds. The results of a late fusion between the best three networks can be seen in the last row. Highlighted in bold are the highest values per column.}
\label{tab:CNN_perform_std}
\end{table}

==> figures/table_variables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l}
\textbf{Clinical variable name}                              & \textbf{Average value negative PCR test} & \textbf{Average value positive PCR test} & \textbf{binary}  \\ 
\hline
incl\_crit\#fever\_or\_chills                                & 0.27                                     & 0.36                                     & yes              \\ 
\hline
incl\_crit\#cough                                            & 0.57                                     & 0.67                                     & yes              \\ 
\hline
incl\_crit\#shortness\_of\_breath\_or\_difficulty\_breathing & 0.93                                     & 0.94                                     & yes              \\ 
\hline
incl\_crit\#loss\_of\_taste                                  & 0.0                                      & 0.09                                     & yes              \\ 
\hline
incl\_crit\#loss\_of\_smell                                  & 0.03                                     & 0.06                                     & yes              \\ 
\hline
incl\_crit\#sore\_throat                                     & 0.03                                     & 0.03                                     & yes              \\ 
\hline
incl\_crit\#congestion                                       & 0.0                                      & 0.0                                      & no               \\ 
\hline
incl\_crit\#runny\_nose                                      & 0.07                                     & 0.03                                     & yes              \\ 
\hline
dur\_symp                                                    & 13.38                                    & 8.12                                     & no               \\ 
\hline
pat\_birth\_year                                             & 1956.87                                  & 1954.79                                  & no               \\ 
\hline
pat\_sex                                                     & 0.73                                     & 0.58                                     & yes              \\ 
\hline
pat\_height                                                  & 173.7                                    & 169.81                                   & no               \\ 
\hline
pat\_weight                                                  & 81.47                                    & 81.15                                    & no               \\ 
\hline
pat\_bmi                                                     & 27.04                                    & 28.3                                     & no               \\ 
\hline
patient\_symp\#Fever                                         & 0.27                                     & 0.39                                     & yes              \\ 
\hline
patient\_symp\#Coughing                                      & 0.53                                     & 0.73                                     & yes              \\ 
\hline
patient\_symp\#Sore\_throat                                  & 0.03                                     & 0.06                                     & yes              \\ 
\hline
patient\_symp\#Running\_nose                                 & 0.1                                      & 0.03                                     & yes              \\ 
\hline
patient\_symp\#Earache                                       & 0.0                                      & 0.0                                      & no               \\ 
\hline
patient\_symp\#Wheezing                                      & 0.0                                      & 0.0                                      & no               \\ 
\hline
patient\_symp\#Chest\_pain                                   & 0.33                                     & 0.15                                     & yes              \\ 
\hline
patient\_symp\#Muscle\_pain                                  & 0.0                                      & 0.18                                     & yes              \\ 
\hline
patient\_symp\#Joint\_pain                                   & 0.0                                      & 0.03                                     & yes              \\ 
\hline
patient\_symp\#Fatigue                                       & 0.1                                      & 0.3                                      & yes              \\ 
\hline
patient\_symp\#Dyspnea                                       & 0.87                                     & 0.91                                     & yes              \\ 
\hline
patient\_symp\#Headache                                      & 0.07                                     & 0.15                                     & yes              \\ 
\hline
patient\_symp\#Decreased\_consciousness                      & 0.03                                     & 0.0                                      & yes              \\ 
\hline
patient\_symp\#Confusion                                     & 0.0                                      & 0.09                                     & yes              \\ 
\hline
patient\_symp\#Abdominal\_pain                               & 0.1                                      & 0.0                                      & yes              \\ 
\hline
patient\_symp\#Nausea                                        & 0.23                                     & 0.12                                     & yes              \\ 
\hline
patient\_symp\#Vomitting                                     & 0.13                                     & 0.12                                     & yes              \\ 
\hline
patient\_symp\#Diarrhea                                      & 0.07                                     & 0.15                                     & yes              \\ 
\hline
patient\_symp\#Skin\_rash                                    & 0.0                                      & 0.0                                      & no               \\ 
\hline
patient\_symp\#Lymphadenopathy                               & 0.0                                      & 0.0                                      & no               \\ 
\hline
patient\_symp\#AgeusiaDysgeusia                              & 0.0                                      & 0.12                                     & yes              \\ 
\hline
patient\_symp\#AnosmiaHyposmia                               & 0.03                                     & 0.09                                     & yes              \\ 
\hline
oxygen\_saturation\_without\_ox                              & 94.67                                    & 90.64                                    & no               \\ 
\hline
respiratory\_rate                                            & 19.33                                    & 22.53                                    & no               \\ 
\hline
pulse                                                        & 89.83                                    & 95.12                                    & no               \\ 
\hline
body\_temperature                                            & 36.99                                    & 37.51                                    & no               \\ 
\hline
emerg\_case\#Yes                                             & 1.0                                      & 0.97                                     & yes              \\ 
\hline
hist\_pulm\_dis                                              & 0.57                                     & 0.58                                     & yes              \\ 
\hline
applying\_pulm\_dis\#Asthma\_bronchiale                      & 0.03                                     & 0.12                                     & yes              \\ 
\hline
applying\_pulm\_dis\#COPD                                    & 0.23                                     & 0.18                                     & yes              \\ 
\hline
applying\_pulm\_dis\#Pneumonia                               & 0.1                                      & 0.12                                     & yes              \\ 
\hline
applying\_pulm\_dis\#Interstitial\_Lung\_Disease             & 0.0                                      & 0.03                                     & yes              \\ 
\hline
applying\_pulm\_dis\#Diffuse\_Parenchymal\_Lung\_Disease     & 0.0                                      & 0.0                                      & no               \\ 
\hline
applying\_pulm\_dis\#Cystic\_fibrosis                        & 0.0                                      & 0.0                                      & no               \\ 
\hline
applying\_pulm\_dis\#Pneumothorax                            & 0.0                                      & 0.0                                      & no               \\ 
\hline
applying\_pulm\_dis\#Tuberculosis                            & 0.0                                      & 0.0                                      & no               \\ 
\hline
applying\_pulm\_dis\#Dyspnea                                 & 0.03                                     & 0.0                                      & yes              \\ 
\hline
applying\_pulm\_dis\#Other                                   & 0.07                                     & 0.0                                      & yes              \\ 
\hline
smok\_years                                                  & 37.45                                    & 41.78                                    & no               \\ 
\hline
pH\_find                                                     & 7.45                                     & 7.47                                     & no               \\ 
\hline
pCO2\_find                                                   & 4.61                                     & 4.25                                     & no               \\ 
\hline
pO2\_find                                                    & 9.71                                     & 9.29                                     & no               \\ 
\hline
lymphocytes                                                  & 21.31                                    & 14.13                                    & no               \\ 
\hline
HCO3\_find                                                   & 24.11                                    & 23.07                                    & no               \\ 
\hline
excess\_find                                                 & 0.55                                     & 0.16                                     & no               \\ 
\hline
hg\_find                                                     & 7.46                                     & 8.43                                     & no               \\ 
\hline
trombocytes\_find                                            & 248.03                                   & 217.6                                    & no               \\ 
\hline
leucocytes\_find                                             & 11.5                                     & 7.37                                     & no               \\ 
\hline
LDH\_find                                                    & 239.79                                   & 379.16                                   & no               \\ 
\hline
CRP                                                          & 51.23                                    & 110.36                                   & no               \\ 
\hline
sys\_bp                                                      & 128.47                                   & 132.7                                    & no               \\ 
\hline
dias\_bp                                                     & 77.23                                    & 79.09                                    & no              
\end{tabular}
}
\caption{Clinical variables that were picked for further analysis. For binary variables 1 = yes and 0 = no.}
\label{tab:feat_summ}
\end{table}


==> table_std.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l|l|l|l}
Model          & \multicolumn{3}{c|}{Images}                                                                              & \multicolumn{3}{c|}{Images and Features}                                                        & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Images and Features \\ without Blood Test\end{tabular}}  \\ 
\hline
               & accuracy                               & sensitivity                    & specificity                    & accuracy                       & sensitivity                   & specificity                    & accuracy                      & sensitivity                    & specificity                           \\ 
\hline
POCOVID-Net         & \textbf{73.4\%±5}                      & \textbf{0.90±0.13}             & 0.55±0.24                      & 78.4\%±9                       & 0.87±0.12                     & 0.69±0.19                      & 78.4\%±8                      & 0.77±0.14                      & 0.8±0.12                              \\ 
\hline
ResNet50       & 63.2\%±14                              & 0.77±0.33                      & 0.50±0.35                      & \textbf{80.3\%±13}             & 0.67±0.3                      & \textbf{0.93±0.08}             & \textbf{83.4\%±5}             & \textbf{0.84±0.01}             & 0.83±0.11                             \\ 
\hline
NASNetMobile   & 58.2\%±7                               & 0.61±0.25                      & \textbf{0.90±0.13}             & 78.5\%±17                      & 0.67±0.3                      & 0.9±0.13                       & 75.0\%±17                     & 0.6±0.38                       & \textbf{0.89±0.09}                    \\ 
\hline
MobileNetV2    & 68.4\%±10                              & 0.64±0.2                       & 0.73±0.13                      & 78.4\%±9                       & \textbf{0.88±0.15}            & 0.69±0.22                      & 78.3\%±13                     & 0.7±0.2                        & 0.87±0.12                             \\ 
\hline
EfficientNetB7 & 71.7\%±9                               & 0.77±0.17                      & 0.65±0.25                      & 76.3\%±10                      & 0.64±0.2                      & 0.89±0.09                      & 76.8\%±9                      & 0.81±0.12                      & 0.73±0.27                             \\ 
%\hline
% Late fusion    & \multicolumn{1}{c|}{\textbf{75.2\%±8}} & \multicolumn{1}{c|}{0.84±0.15} & \multicolumn{1}{c|}{0.65±0.25} & \multicolumn{1}{c|}{76.9\%±16} & \multicolumn{1}{c|}{0.67±0.3} & \multicolumn{1}{c|}{0.87±0.12} & \multicolumn{1}{c|}{80.1\%±8} & \multicolumn{1}{c|}{0.77±0.14} & \multicolumn{1}{c}{0.83±0.11}        
\bottomrule
\end{tabular}
}
\caption{Performance of different network architectures on the three configurations of the dataset together with the standard deviation over the five folds. The results of a late fusion between the best three networks can be seen in the last row. Highlighted in bold are the highest values per column.}
\label{tab:CNN_perform_std}
\end{table}

